A Non-linear GPU Thread Map for Triangular Domains

There is a stage in the GPU computing pipeline where a grid of thread-blocks, in \textit{parallel space}, is mapped onto the problem domain, in \textit{data space}. Since the parallel space is restricted to a box type geometry, the mapping approach is typically a $k$-dimensional bounding box (BB) that covers a $p$-dimensional data space. Threads that fall inside the domain perform computations while threads that fall outside are discarded at runtime. In this work we study the case of mapping threads efficiently onto triangular domain problems and propose a block-space linear map $\lambda(\omega)$, based on the properties of the lower triangular matrix, that reduces the number of unnnecessary threads from $\mathcal{O}(n^2)$ to $\mathcal{O}(n)$. Performance results for global memory accesses show an improvement of up to $18\%$ with respect to the \textit{bounding-box} approach, placing $\lambda(\omega)$ on second place below the \textit{rectangular-box} approach and above the \textit{recursive-partition} and \textit{upper-triangular} approaches. For shared memory scenarios $\lambda(\omega)$ was the fastest approach achieving $7\%$ of performance improvement while preserving thread locality. The results obtained in this work make $\lambda(\omega)$ an interesting map for efficient GPU computing on parallel problems that define a triangular domain with or without neighborhood interactions. The extension to tetrahedral domains is analyzed, with applications to triplet-interaction n-body applications.

==> plots/genplot_bestimp <==
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 26
set output 'bestimp.eps'
#set ylabel 'I'
#set ylabel rotate right
set label 1 'I' at graph -0.15, graph 0.55
set xlabel 'N (2^10)'
set xtics font "Times, 20"
set ytics font "Times, 20"
set title 'Performance of square root strategies'
f(x) = a*x + b
g(x) = c*x + d
h(x) = s*x + u
set key box linestyle 1 lc rgb "black" maxrows 3 width -6.0
set key Left samplen 1.0 reverse  
set key spacing 0.7 font "Times, 14" 
set pointsize 0.8
set style line 3 linewidth 1.0
set xrange [0:32]

plot	'../results_GTX680/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$5) 	title 'LTM-R@GTX680'	 		with linespoints pt 6 lt 3 lc rgb "red",\
		'../results_TeslaK40/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$2) notitle 				with lines ls 1 lc rgb "black",\
		'../results_GTX680/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$4) 	title 'LTM-N@GTX680'	 		with linespoints ls 3 pt 6 lc rgb "blue",\
		'../results_GTX680/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$3) 	title 'LTM-X@GTX680'	 		with linespoints ls 3 pt 6 lc rgb "magenta",\
		'../results_GTX765M/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$5) 	title 'LTM-R@GTX765M'	  		with linespoints ls 3 pt 8 lc rgb "red",\
		'../results_GTX765M/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$4) 	title 'LTM-N@GTX765M' 			with linespoints ls 3 pt 8 lc rgb "blue",\
		'../results_GTX765M/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$3) 	title 'LTM-X@GTX765M' 			with linespoints ls 3 pt 8 lc rgb "magenta",\
		'../results_TeslaK40/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$3) title 'LTM-X@TeslaK40' 	 		with linespoints ls 3 pt 2 lc rgb "magenta",\
		'../results_TeslaK40/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$4) title 'LTM-N@TeslaK40' 	 		with linespoints ls 3 pt 2 lc rgb "blue",\
		'../results_TeslaK40/dummy_results/full_implementation_results.dat' using ($1/1000):($2/$5) title 'LTM-R@TeslaK40' 	 		with linespoints ls 3 pt 2 lc rgb "red"


==> plots/genplot_blocks <==
# Gnuplot script file for plotting data in file "worst_case.dat"
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 26
set output 'wasted_blocks.eps'
set ylabel '# blocks'
set xlabel 'N (2^10)'
set xtics font "Times, 20"
set ytics font "Times, 20"
set title 'Wasted blocks'
set key box linestyle 1 lc rgb "black" left Left reverse samplen 1 width 1.0
set key spacing 1.0 font "Times, 14"
set pointsize 0.8
set style line 1 lw 0.5
set log y
#set format y "%1.0e"
B = 16
set xrange [0:32]
plot 	"td1_data.dat" using ($1/1000):(ceil(($1/B)*(($1/B)+1)/2)) title 'BB' with linespoints lt 1 pt 2 lc rgb "black", \
 		"td3_data.dat" using ($1/1000):(ceil(($1/(B*2)))) title 'LTM' with linespoints lt 1 pt 6 lc rgb "red"
reset


==> plots/genplot_collision1d <==
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 20
set output 'collision1d.eps'
#set ylabel 't/BB'
#set ylabel rotate right
set xlabel 'N (2^10)'
set label 1 'I' at graph -0.1, graph 0.55
set xtics font "Times, 18"
set ytics font "Times, 18"
set title '1D Collision Detection'
set key box linestyle 1 lc rgb "black" maxrows 4 
set key Left right top samplen 0.5 reverse width -1.5
set key spacing 1.0 font "Times, 17" 
set pointsize 1.0
set style line 3 linewidth 1.0
set xrange [1:32]

plot	'../results_GTX765M/collision1d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "brown",\
		'../results_GTX765M/collision1d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX765M'			with linespoints ls 3 pt 8 lc rgb "blue",\
		'../results_GTX765M/collision1d_results/full_results.dat' using ($1/1000):($2/$2) notitle 					with lines ls 1 lc rgb "black",\
		'../results_GTX765M/collision1d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "red",\
		'../results_GTX765M/collision1d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX765M'			with linespoints ls 3 pt 8 lc rgb "magenta",\
\
		'../results_GTX680/collision1d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "brown",\
		'../results_GTX680/collision1d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX680'			with linespoints ls 3 pt 6 lc rgb "blue",\
		'../results_GTX680/collision1d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "red",\
		'../results_GTX680/collision1d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX680'			with linespoints ls 3 pt 6 lc rgb "magenta",\
\
		'../results_TeslaK40/collision1d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "brown",\
		'../results_TeslaK40/collision1d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "blue",\
		'../results_TeslaK40/collision1d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "red",\
		'../results_TeslaK40/collision1d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "magenta"


==> plots/genplot_collision2d <==
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 26
set output 'collision2d.eps'
#set ylabel 't/BB'
#set ylabel rotate right
set xlabel 'N'
#set ylabel 'I'
#set log y
set label 1 'I' at graph -0.1, graph 0.55
set xtics font "Times, 20"
set ytics font "Times, 20"
set title '2D Collision Detection'
set key box linestyle 1 lc rgb "black" maxrows 4 
set key Left right top samplen 0.5 reverse width -6.0
set key spacing 0.6 font "Times, 12" 
set pointsize 0.6
set style line 3 linewidth 1.0

plot	'../results_GTX765M/collision2d_results/full_results.dat' using 1:($2/$6) title 'AVRIL@GTX765M'		with linespoints ls 3 pt 8 lc rgb "brown",\
		'../results_GTX765M/collision2d_results/full_results.dat' using 1:($2/$5) title 'REC@GTX765M'			with linespoints ls 3 pt 8 lc rgb "blue",\
		'../results_GTX765M/collision2d_results/full_results.dat' using 1:($2/$2) notitle 					with lines ls 1 lc rgb "black",\
		'../results_GTX765M/collision2d_results/full_results.dat' using 1:($2/$3) title 'RSQRT@GTX765M'		with linespoints ls 3 pt 8 lc rgb "red",\
		'../results_GTX765M/collision2d_results/full_results.dat' using 1:($2/$4) title 'RB@GTX765M'			with linespoints ls 3 pt 8 lc rgb "magenta",\
\
		'../results_GTX680/collision2d_results/full_results.dat' using 1:($2/$6) title 'AVRIL@GTX680'			with linespoints ls 3 pt 6 lc rgb "brown",\
		'../results_GTX680/collision2d_results/full_results.dat' using 1:($2/$5) title 'REC@GTX680'			with linespoints ls 3 pt 6 lc rgb "blue",\
		'../results_GTX680/collision2d_results/full_results.dat' using 1:($2/$3) title 'RSQRT@GTX680'			with linespoints ls 3 pt 6 lc rgb "red",\
		'../results_GTX680/collision2d_results/full_results.dat' using 1:($2/$4) title 'RB@GTX680'			with linespoints ls 3 pt 6 lc rgb "magenta",\
\
		'../results_TeslaK40/collision2d_results/full_results.dat' using 1:($2/$6) title 'AVRIL@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "brown",\
		'../results_TeslaK40/collision2d_results/full_results.dat' using 1:($2/$5) title 'REC@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "blue",\
		'../results_TeslaK40/collision2d_results/full_results.dat' using 1:($2/$3) title 'RSQRT@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "red",\
		'../results_TeslaK40/collision2d_results/full_results.dat' using 1:($2/$4) title 'RB@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "magenta",\
		'../results_TeslaK40/collision2d_results/full_results.dat' using 1:($2/$3) notitle	with linespoints ls 3 pt 2 lc rgb "red",\


==> plots/genplot_collision3d <==
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 20
set output 'collision3d.eps'
#set ylabel 't/BB'
#set ylabel rotate right
set xlabel 'N (2^10)'
set label 1 'I' at graph -0.1, graph 0.55
set xtics font "Times, 18"
set ytics font "Times, 18"
set title '3D Collision Detection'
set key box linestyle 1 lc rgb "black" maxrows 4 
set key Left right top samplen 0.5 reverse width -1.5
set key spacing 1.0 font "Times, 17" 
set pointsize 1.0
set style line 3 linewidth 1.0
set xrange [1:32]

plot	'../results_GTX765M/collision3d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "brown",\
		'../results_GTX765M/collision3d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX765M'			with linespoints ls 3 pt 8 lc rgb "blue",\
		'../results_GTX765M/collision3d_results/full_results.dat' using ($1/1000):($2/$2) notitle 					with lines ls 1 lc rgb "black",\
		'../results_GTX765M/collision3d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "red",\
		'../results_GTX765M/collision3d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX765M'			with linespoints ls 3 pt 8 lc rgb "magenta",\
\
		'../results_GTX680/collision3d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "brown",\
		'../results_GTX680/collision3d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX680'			with linespoints ls 3 pt 6 lc rgb "blue",\
		'../results_GTX680/collision3d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "red",\
		'../results_GTX680/collision3d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX680'			with linespoints ls 3 pt 6 lc rgb "magenta",\
\
		'../results_TeslaK40/collision3d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "brown",\
		'../results_TeslaK40/collision3d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "blue",\
		'../results_TeslaK40/collision3d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "red",\
		'../results_TeslaK40/collision3d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "magenta"


==> plots/genplot_dummy <==
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 20
set output 'dummy.eps'
#set ylabel 't/BB'
#set ylabel rotate right
set xlabel 'N (2^10)'
#set ylabel 'I'
set label 1 'I' at graph -0.1, graph 0.55
set xtics font "Times, 18"
set ytics font "Times, 18"
set title 'Dummy Kernel'
set key box linestyle 1 lc rgb "black" maxrows 4 
set key Left right bottom samplen 0.5 reverse width -1.5
set key spacing 1.0 font "Times, 17" 
set pointsize 1.0
set style line 3 linewidth 1.0
set xrange [1:32]

plot		'../results_GTX765M/dummy_results/full_results.dat' using ($1/1000):($2/$2) notitle 					with lines ls 1 lc rgb "black",\
\
		'../results_GTX765M/dummy_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "brown",\
		'../results_GTX765M/dummy_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX765M'			with linespoints ls 3 pt 8 lc rgb "blue",\
		'../results_GTX765M/dummy_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "red",\
		'../results_GTX765M/dummy_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX765M'			with linespoints ls 3 pt 8 lc rgb "magenta",\
\
		'../results_GTX680/dummy_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "brown",\
		'../results_GTX680/dummy_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX680'			with linespoints ls 3 pt 6 lc rgb "blue",\
		'../results_GTX680/dummy_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "red",\
		'../results_GTX680/dummy_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX680'			with linespoints ls 3 pt 6 lc rgb "magenta",\
\
		'../results_TeslaK40/dummy_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "brown",\
		'../results_TeslaK40/dummy_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "blue",\
		'../results_TeslaK40/dummy_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "red",\
		'../results_TeslaK40/dummy_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "magenta"


==> plots/genplot_edm4d <==
set   autoscale                        # scale axes automatically
set term postscript eps color blacktext "Times" 20
set output 'edm4d.eps'
#set ylabel 't/BB'
#set ylabel rotate right
set xlabel 'N (2^10)'

set label 1 'I' at graph -0.1, graph 0.55
set xtics font "Times, 18"
set ytics font "Times, 18"
set title 'EDM 4D'
set key box linestyle 1 lc rgb "black" maxrows 4 
set key Left right bottom samplen 0.5 reverse width -1.5
set key spacing 1.0 font "Times, 17" 
set pointsize 1.0
set style line 3 linewidth 1.0
set xrange [1:32]

plot	'../results_GTX765M/edm4d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "brown",\
		'../results_GTX765M/edm4d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX765M'			with linespoints ls 3 pt 8 lc rgb "blue",\
		'../results_GTX765M/edm4d_results/full_results.dat' using ($1/1000):($2/$2) notitle 					with lines ls 1 lc rgb "black",\
		'../results_GTX765M/edm4d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX765M'		with linespoints ls 3 pt 8 lc rgb "red",\
		'../results_GTX765M/edm4d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX765M'			with linespoints ls 3 pt 8 lc rgb "magenta",\
\
		'../results_GTX680/edm4d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "brown",\
		'../results_GTX680/edm4d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@GTX680'			with linespoints ls 3 pt 6 lc rgb "blue",\
		'../results_GTX680/edm4d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@GTX680'			with linespoints ls 3 pt 6 lc rgb "red",\
		'../results_GTX680/edm4d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@GTX680'			with linespoints ls 3 pt 6 lc rgb "magenta",\
\
		'../results_TeslaK40/edm4d_results/full_results.dat' using ($1/1000):($2/$6) title 'UTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "brown",\
		'../results_TeslaK40/edm4d_results/full_results.dat' using ($1/1000):($2/$5) title 'REC@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "blue",\
		'../results_TeslaK40/edm4d_results/full_results.dat' using ($1/1000):($2/$3) title 'LTM@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "red",\
		'../results_TeslaK40/edm4d_results/full_results.dat' using ($1/1000):($2/$4) title 'RB@TeslaK40'		with linespoints ls 3 pt 2 lc rgb "magenta"

